Enriching Biomedical Knowledge for Low-resource Language Through Large-Scale Translation

Biomedical data and benchmarks are highly valuable yet very limited in low-resource languages other than English such as Vietnamese. In this paper, we make use of a state-of-the-art translation model in English-Vietnamese to translate and produce both pretrained as well as supervised data in the biomedical domains. Thanks to such large-scale translation, we introduce ViPubmedT5, a pretrained Encoder-Decoder Transformer model trained on 20 million translated abstracts from the high-quality public PubMed corpus. ViPubMedT5 demonstrates state-of-the-art results on two different biomedical benchmarks in summarization and acronym disambiguation. Further, we release ViMedNLI - a new NLP task in Vietnamese translated from MedNLI using the recently public En-vi translation model and carefully refined by human experts, with evaluations of existing methods against ViPubmedT5.

==> sections/figure/vimednli_process.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth,keepaspectratio]{sections/figure/vimednli_process.drawio.pdf}
    \caption{The Process of ViMedNLI Corpus Creation}
    \label{fig:vipubmedt5}
\end{figure}

==> sections/tables/acextable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[hbt!]
\centering
\caption{Some Examples of Abbreviations Refining}

% \begin{tabular}{@{}l|l|l|l@{}}
% \toprule
% \# & MedNLI                                                                            & Translated by NMT                                                                   & Our Refined                                                                               \\ \midrule
% 1  & \begin{tabular}[c]{@{}l@{}}the patient has no \\ history of \colorbox{green}{GI bleed}\end{tabular} & \begin{tabular}[c]{@{}l@{}}bệnh nhân không có \\ tiền sử xuất huyết GI\end{tabular} & \begin{tabular}[c]{@{}l@{}}bệnh nhân không có tiền sử xuất\\  huyết tiêu hóa\end{tabular} \\ \midrule
% 2  & \begin{tabular}[c]{@{}l@{}}the patient has no\\  history of GI bleed\end{tabular} & \begin{tabular}[c]{@{}l@{}}bệnh nhân không có \\ tiền sử xuất huyết GI\end{tabular} & \begin{tabular}[c]{@{}l@{}}bệnh nhân không có tiền sử \\ \colorbox{green}{xuất huyết tiêu hóa}\end{tabular} \\ \midrule
% 2  & \begin{tabular}[c]{@{}l@{}}the patient has no \\ history of GI bleed\end{tabular} & \begin{tabular}[c]{@{}l@{}}bệnh nhân không có \\ tiền sử xuất huyết GI\end{tabular} & \begin{tabular}[c]{@{}l@{}}bệnh nhân không có tiền sử \\ xuất huyết tiêu hóa\end{tabular} \\ \bottomrule
% \end{tabular}

\begin{tabular}{ll|l|l}
\hline
\textbf{\#} & \textbf{MedNLI}                                                                           & \textbf{Translated by NMT}                                                                   & \textbf{Our Refined}                                                                                 \\ \hline
1           & \begin{tabular}[c]{@{}l@{}}Electrocardiograms \\ revealed no \\ \colorbox{green}{QRS} changes.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Điện tâm đồ cho thấy \\ không có thay đổi về \\ \colorbox{yellow}{QRS}.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Điện tâm đồ cho thấy \\ không có thay đổi về\\  \colorbox{yellow}{phức độ QRS}.\end{tabular} \\ \hline
2           & \begin{tabular}[c]{@{}l@{}}Patient has \\ no \colorbox{green}{PMH}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Bệnh nhân \\ không có \colorbox{yellow}{PMH}\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}Bệnh nhân \\ \colorbox{yellow}{không có tiền sử bệnh}\end{tabular}                           \\ \hline
3           & \begin{tabular}[c]{@{}l@{}}Patient is\\  \colorbox{green}{post op}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Bệnh nhân đã \\ \colorbox{yellow}{hồi phục} \textit{(Patient is recovered)}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Bệnh nhân\\ \colorbox{yellow}{hậu phẫu thuật}
\end{tabular}                                   \\ \hline

% 3           & \begin{tabular}[c]{@{}l@{}}Patient is\\  \colorbox{green}{post op}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Bệnh nhân đã \\ \colorbox{yellow}{hồi phục} \textit{(Patient is recovered)}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Bệnh nhân\\ \colorbox{yellow}{hậu phẫu thuật}
% \end{tabular}                                   \\ \hline


% The patient had an sotesophytes

\end{tabular}


\begin{tablenotes}
      % \small
      % \large
      \item \textit{\#1:} Abbreviation in English can be used in both English and Vietnamese
      \item \textit{\#2:} Abbreviation can only be used in English. In Vietnamese, abbreviation is different.
      \item \textit{\#3:} Abbreviation  in English is wrong when translated to Vietnamese
\end{tablenotes}
\label{ac_ex_table}

\end{table*}
